Enhancing Intrinsic Features for Debiasing via Investigating Class-Discerning Common Attributes in Bias-Contrastive Pair

In the image classification task, deep neural networks frequently rely on bias attributes that are spuriously correlated with a target class in the presence of dataset bias, resulting in degraded performance when applied to data without bias attributes. The task of debiasing aims to compel classifiers to learn intrinsic attributes that inherently define a target class rather than focusing on bias attributes. While recent approaches mainly focus on emphasizing the learning of data samples without bias attributes (i.e., bias-conflicting samples) compared to samples with bias attributes (i.e., bias-aligned samples), they fall short of directly guiding models where to focus for learning intrinsic features. To address this limitation, this paper proposes a method that provides the model with explicit spatial guidance that indicates the region of intrinsic features. We first identify the intrinsic features by investigating the class-discerning common features between a bias-aligned (BA) sample and a bias-conflicting (BC) sample (i.e., bias-contrastive pair). Next, we enhance the intrinsic features in the BA sample that are relatively under-exploited for prediction compared to the BC sample. To construct the bias-contrastive pair without using bias information, we introduce a bias-negative score that distinguishes BC samples from BA samples employing a biased model. The experiments demonstrate that our method achieves state-of-the-art performance on synthetic and real-world datasets with various levels of bias severity.

==> table/auxdata_analysis_wstd.tex <==
% \begin{table}[t!]
% \centering
% % \vspace{0.05cm}
% % \caption{
% % The remaining number of bias-aligned samples~(\# of B.A.) and bias-conflicting ones~(\# of B.C.) in the bias-amplified dataset $\mathcal{D}_A$ after applying BE.
% % % $M$ indicates the number of BCDs.
% % The remaining numbers are shown in ratios of samples compared to the original training dataset $\mathcal{D}$.}
% \caption{The number of remaining bias-aligned samples (\# of B.A.) and bias-conflicting ones~(\# of B.C.) depending on sampling methods. The last column of each dataset represents the ratio of \# of B.A. to \# of B.C. }
% % \vspace{-0.1cm}
% % and evaluated on the same bias severity setting (1.0\%).}
% \resizebox{1.0\linewidth}{!}{
% \setlength{\tabcolsep}{0.7em}
% % \setlength{\tabcolsep}{0.3em}
% % \def\arraystretch{1.2}% 
% \begin{tabular}{ c | c c | c c}
% % \hline\noalign{\smallskip}
% \toprule 

% % Method & $\rho$ & $M$ & Colored MNIST & BFFHQ & Dogs \& Cats & BAR \\
% % \multicolumn{1}{c|}{\multirow{2}{*}{Method}}
% % \multicolumn{1}{c}{\multirow{2}{*}{$\rho$}}
% \multicolumn{1}{c|}{\multirow{2}{*}{}}
% & \multicolumn{2}{c}{Waterbirds}
% & \multicolumn{2}{c}{BFFHQ}
% \\ \cmidrule(lr){2-3}\cmidrule(lr){4-5}
% % \\ \midrule
% % \multicolumn{3}{c}{}
% & B.A. $\downarrow$ & B.C. $\uparrow$ & B.A. $\downarrow$ & B.C. $\uparrow$ \\     
% \midrule
% $\mathcal{D}_\text{C}$  
% & 163.8\stdv{20.56} & 39.0\stdv{1.41}
% & 286.8\stdv{47.57} & 104.0\stdv{1.41} \\
% \midrule
% \multirow{2}{*}{$\mathcal{D}_\text{aux}$}   
% & 134.4\stdv{15.35} &   38.0\stdv{1.67}
% & 87.0\stdv{16.8} & 96.0\stdv{2.0} \\
% %  & \cellcolor{Gray}(-29.4) & \cellcolor{Gray}(-1.0) 
% %  & \cellcolor{Gray}(-199.8) & \cellcolor{Gray}(-8.0)\\
% %  \midrule
% % $\mathcal{D}_\text{aux}$ 
% & \cellcolor{Gray}2.83\%\stdv{0.32} & \cellcolor{Gray}79.1\%\stdv{3.48} 
% & \cellcolor{Gray}0.45\%\stdv{0.08} & \cellcolor{Gray}50.0\%\stdv{1.04} \\
% \bottomrule
% \end{tabular}}
% % \vspace{-0.5cm}
% \label{tab:auxcomposition}
% \end{table}


% \begin{table}[t!]
% \centering
% % \vspace{0.05cm}
% % \caption{
% % The remaining number of bias-aligned samples~(\# of B.A.) and bias-conflicting ones~(\# of B.C.) in the bias-amplified dataset $\mathcal{D}_A$ after applying BE.
% % % $M$ indicates the number of BCDs.
% % The remaining numbers are shown in ratios of samples compared to the original training dataset $\mathcal{D}$.}
% \caption{The number of remaining bias-aligned samples (\# of B.A.) and bias-conflicting ones~(\# of B.C.) depending on sampling methods. The last column of each dataset represents the ratio of \# of B.A. to \# of B.C. }
% % \vspace{-0.1cm}
% % and evaluated on the same bias severity setting (1.0\%).}
% \resizebox{1.0\linewidth}{!}{
% \setlength{\tabcolsep}{0.3em}
% \def\arraystretch{1.5}% 
% \begin{tabular}{ c | c c c | c c c}
% % \hline\noalign{\smallskip}
% \toprule 

% % Method & $\rho$ & $M$ & Colored MNIST & BFFHQ & Dogs \& Cats & BAR \\
% % \multicolumn{1}{c|}{\multirow{2}{*}{Method}}
% % \multicolumn{1}{c}{\multirow{2}{*}{$\rho$}}
% \multicolumn{1}{c|}{\multirow{2}{*}{}}

% % & \multicolumn{3}{c}{\# of B.C. $\uparrow$}
% & $\mathcal{D}_\text{C}$  & \multicolumn{2}{c}{$\mathcal{D}_\text{aux}$}
% & $\mathcal{D}_\text{C}$  & \multicolumn{2}{c}{$\mathcal{D}_\text{aux}$} 
% \\ \cmidrule(lr){2-2} \cmidrule(lr){3-4} \cmidrule(lr){5-5} \cmidrule(lr){6-7}
% % \\ \midrule
% % \multicolumn{3}{c}{}

% Dataset   
% % & {\# of B.A. $\downarrow$}
% % & {\# of B.A. $\downarrow$}
% % & {\% of B.A. $\downarrow$}
% % & {\# of B.C. $\uparrow$}
% % & {\# of B.C. $\uparrow$}
% % & {\% of B.C. $\uparrow$}
% & {B.A. (\#) $\downarrow$} 
% & {B.A. (\#) $\downarrow$} 
% & {B.A. (\%) $\downarrow$}
% & {B.C. (\#) $\uparrow$} 
% & {B.C. (\#) $\uparrow$} 
% & {B.C. (\%) $\uparrow$}
% \\
% \midrule
% Waterbirds 
% & 163.8\stdv{20.56}
% & 134.4\stdv{15.35}
% & \cellcolor{Gray}2.83\stdv{0.32}

% & 39.0\stdv{1.41}
% & 38.0\stdv{1.67}
% & \cellcolor{Gray}79.1\stdv{3.48}
% \\

% BFFHQ 
% & 286.8\stdv{47.57}
% & 87.0\stdv{16.8}
% & \cellcolor{Gray}0.45\stdv{0.08}

% & 104.0\stdv{1.41}
% & 96.0\stdv{2.0}
% & \cellcolor{Gray}50.0\stdv{1.04}
% \\

% \bottomrule
% \end{tabular}}

% % \vspace{-0.5cm}
% \label{tab:auxcomposition}
% \end{table}

% \begin{table}[t!]
% \centering
% % \vspace{0.05cm}
% % \caption{
% % The remaining number of bias-aligned samples~(\# of B.A.) and bias-conflicting ones~(\# of B.C.) in the bias-amplified dataset $\mathcal{D}_A$ after applying BE.
% % % $M$ indicates the number of BCDs.
% % The remaining numbers are shown in ratios of samples compared to the original training dataset $\mathcal{D}$.}
% \caption{The number of remaining bias-aligned samples (\# of B.A.) and bias-conflicting ones~(\# of B.C.) depending on sampling methods. The last column of each dataset represents the ratio of \# of B.A. to \# of B.C. }
% % \vspace{-0.1cm}
% % and evaluated on the same bias severity setting (1.0\%).}
% \resizebox{1.0\linewidth}{!}{
% \setlength{\tabcolsep}{0.2em}
% \def\arraystretch{1.2}% 
% \begin{tabular}{ c | c c c | c c c}
% % \hline\noalign{\smallskip}
% \toprule 

% % Method & $\rho$ & $M$ & Colored MNIST & BFFHQ & Dogs \& Cats & BAR \\
% % \multicolumn{1}{c|}{\multirow{2}{*}{Method}}
% % \multicolumn{1}{c}{\multirow{2}{*}{$\rho$}}
% \multicolumn{1}{c|}{\multirow{2}{*}{}}

% % & \multicolumn{3}{c}{\# of B.C. $\uparrow$}
% & $\mathcal{D}_\text{C}$  & \multicolumn{2}{c}{$\mathcal{D}_\text{aux}$}
% & $\mathcal{D}_\text{C}$  & \multicolumn{2}{c}{$\mathcal{D}_\text{aux}$} 
% \\ \cmidrule(lr){2-2} \cmidrule(lr){3-4} \cmidrule(lr){5-5} \cmidrule(lr){6-7}
% % \\ \midrule
% % \multicolumn{3}{c}{}

% Dataset   
% % & {\# of B.A. $\downarrow$}
% % & {\# of B.A. $\downarrow$}
% % & {\% of B.A. $\downarrow$}
% % & {\# of B.C. $\uparrow$}
% % & {\# of B.C. $\uparrow$}
% % & {\% of B.C. $\uparrow$}
% & {B.A. (\#) $\downarrow$} 
% & {B.A. (\#) $\downarrow$} 
% & {B.A. (\%) $\downarrow$}
% & {B.C. (\#) $\uparrow$} 
% & {B.C. (\#) $\uparrow$} 
% & {B.C. (\%) $\uparrow$}
% \\
% \midrule
% Waterbirds 
% & 163.8
% & 134.4
% & \cellcolor{Gray}2.83

% & 39.0
% & 38.0
% & \cellcolor{Gray}79.1
% \\

% BFFHQ 
% & 286.8
% & 87.0
% & \cellcolor{Gray}0.45

% & 104.0
% & 96.0
% & \cellcolor{Gray}50.0
% \\

% \bottomrule
% \end{tabular}}

% % \vspace{-0.5cm}
% \label{tab:auxcomposition}
% \end{table}


\begin{table}[t!]
\centering
% \vspace{0.05cm}
% \caption{
% The remaining number of bias-aligned samples~(\# of B.A.) and bias-conflicting ones~(\# of B.C.) in the bias-amplified dataset $\mathcal{D}_A$ after applying BE.
% % $M$ indicates the number of BCDs.
% The remaining numbers are shown in ratios of samples compared to the original training dataset $\mathcal{D}$.}
\caption{The number of remaining bias-aligned samples (\# of B.A.) and bias-conflicting ones~(\# of B.C.) depending on sampling methods. The last column of each dataset represents the ratio of \# of B.A. to \# of B.C. }
% \vspace{-0.1cm}
% and evaluated on the same bias severity setting (1.0\%).}
\resizebox{1.0\linewidth}{!}{
\setlength{\tabcolsep}{0.2em}
\def\arraystretch{1.5}% 
\begin{tabular}{ c | c c c | c c c}
% \hline\noalign{\smallskip}
\toprule 


\multicolumn{1}{c|}{\multirow{2}{*}{}}

& \multicolumn{2}{c}{\# B.A. $\downarrow$}  
&  {\% B.A. $\downarrow$}
& \multicolumn{2}{c}{\# B.C. $\uparrow$} 
&  {\% B.C. $\uparrow$}

% & \multicolumn{2}{c}{B.A. (\#) $\downarrow$}  
% &  {B.A. (\%) $\downarrow$}
% & \multicolumn{2}{c}{B.C. (\#) $\uparrow$} 
% &  {B.C. (\%) $\uparrow$}
\\ \cmidrule(lr){2-3} \cmidrule(lr){4-4} \cmidrule(lr){5-6} \cmidrule(lr){7-7}

Dataset   
% & {\# of B.A. $\downarrow$}
% & {\# of B.A. $\downarrow$}
% & {\% of B.A. $\downarrow$}
% & {\# of B.C. $\uparrow$}
% & {\# of B.C. $\uparrow$}
% & {\% of B.C. $\uparrow$}
& $\mathcal{D}_\text{C}$
& $\mathcal{D}_\text{BN}$
& $\mathcal{D}_\text{BN}$
& $\mathcal{D}_\text{C}$
& $\mathcal{D}_\text{BN}$
& $\mathcal{D}_\text{BN}$

\\
\midrule
Waterbirds 
& 157.00 \stdv{17.25} & 130.50 \stdv{14.79} & \cellcolor{Gray}2.75 \stdv{0.31} 
& 39.00 \stdv{1.58} & 38.25 \stdv{1.79} & \cellcolor{Gray}79.69 \stdv{3.72} \\

BFFHQ 
& 286.80 \stdv{47.57} & 87.00 \stdv{16.89} & \cellcolor{Gray} 0.46 \stdv{0.09} 
& 104.00 \stdv{1.41} & 96.00 \stdv{2.00} & \cellcolor{Gray} 50.00 \stdv{1.04} \\

BAR
& 93.60 \stdv{1.62} & 63.00 \stdv{2.53} & \cellcolor{Gray}3.58 \stdv{0.14} 
& 9.80 \stdv{1.17} & 6.60 \stdv{0.80} & \cellcolor{Gray}47.14 \stdv{5.71} \\
\bottomrule
\end{tabular}}



% \vspace{-0.5cm}
\label{tab:auxcomposition}
\end{table}

% \begin{table}[t!]
% \centering
% % \vspace{0.05cm}
% % \caption{
% % The remaining number of bias-aligned samples~(\# of B.A.) and bias-conflicting ones~(\# of B.C.) in the bias-amplified dataset $\mathcal{D}_A$ after applying BE.
% % % $M$ indicates the number of BCDs.
% % The remaining numbers are shown in ratios of samples compared to the original training dataset $\mathcal{D}$.}
% \caption{The number of remaining bias-aligned samples (\# of B.A.) and bias-conflicting ones~(\# of B.C.) depending on sampling methods. The last column of each dataset represents the ratio of \# of B.A. to \# of B.C. }
% % \vspace{-0.1cm}
% % and evaluated on the same bias severity setting (1.0\%).}
% \resizebox{1.0\linewidth}{!}{
% \setlength{\tabcolsep}{0.2em}
% \def\arraystretch{1.5}% 
% \begin{tabular}{ c | c c | c c}
% % \hline\noalign{\smallskip}
% \toprule 

% % Method & $\rho$ & $M$ & Colored MNIST & BFFHQ & Dogs \& Cats & BAR \\
% % \multicolumn{1}{c|}{\multirow{2}{*}{Method}}
% % \multicolumn{1}{c}{\multirow{2}{*}{$\rho$}}
% \multicolumn{1}{c|}{\multirow{2}{*}{}}

% % & $\mathcal{D}_\text{C}$  & \multicolumn{2}{c}{$\mathcal{D}_\text{aux}$}
% % & $\mathcal{D}_\text{C}$  & \multicolumn{2}{c}{$\mathcal{D}_\text{aux}$} 
% % \\ \cmidrule(lr){2-2} \cmidrule(lr){3-4} \cmidrule(lr){5-5} \cmidrule(lr){6-7}
% & \multicolumn{2}{c}{B.A. $\downarrow$}  
% % &  {B.A. $\downarrow$}
% & \multicolumn{2}{c}{B.C. $\uparrow$} 
% % &  {B.C. $\uparrow$}

% % & \multicolumn{2}{c}{B.A. (\#) $\downarrow$}  
% % &  {B.A. (\%) $\downarrow$}
% % & \multicolumn{2}{c}{B.C. (\#) $\uparrow$} 
% % &  {B.C. (\%) $\uparrow$}
% \\ \cmidrule(lr){2-3}  \cmidrule(lr){4-5} 

% Dataset   
% % & {\# of B.A. $\downarrow$}
% % & {\# of B.A. $\downarrow$}
% % & {\% of B.A. $\downarrow$}
% % & {\# of B.C. $\uparrow$}
% % & {\# of B.C. $\uparrow$}
% % & {\% of B.C. $\uparrow$}
% & $\mathcal{D}_\text{C}$
% & $\mathcal{D}_\text{aux}$
% % & \multicolumn{2}{c}{$\mathcal{D}_\text{aux}$} 
% % & $\mathcal{D}_\text{aux}$
% & $\mathcal{D}_\text{C}$
% & $\mathcal{D}_\text{aux}$
% % & \multicolumn{2}{c}{$\mathcal{D}_\text{aux}$} 
% % & $\mathcal{D}_\text{aux}$

% \\
% \midrule
% Waterbirds 
% & 163.8\stdv{20.56}
% % & 134.4\stdv{15.35} (2.83\%\stdv{0.32}) 
% & $38.0_{\pm{1.67}} (79.1\%_{\pm{3.48}})$ 

% & 39.0\stdv{1.41}
% & $38.0_{\pm{1.67}} (79.1\%_{\pm{3.48}})$ 
% \\

% BFFHQ 
% & 286.8\stdv{47.57}
% % & 87.0\stdv{16.8} (0.45\%\stdv{0.08})
% & $38.0_{\pm{1.67}} (79.1\%_{\pm{3.48}})$ 

% & 104.0\stdv{1.41}
% % & 96.0\stdv{2.0} (50.0\%\stdv{1.04})
% & $38.0_{\pm{1.67}} (79.1\%_{\pm{3.48}})$ 
% \\

% \bottomrule
% \end{tabular}}



% % \vspace{-0.5cm}
% \label{tab:auxcomposition}
% \end{table}

% \begin{table}[t!]
% \centering
% % \vspace{0.05cm}
% % \caption{
% % The remaining number of bias-aligned samples~(\# of B.A.) and bias-conflicting ones~(\# of B.C.) in the bias-amplified dataset $\mathcal{D}_A$ after applying BE.
% % % $M$ indicates the number of BCDs.
% % The remaining numbers are shown in ratios of samples compared to the original training dataset $\mathcal{D}$.}
% \caption{The number of remaining bias-aligned samples (\# of B.A.) and bias-conflicting ones~(\# of B.C.) depending on sampling methods. The last column of each dataset represents the ratio of \# of B.A. to \# of B.C. }
% % \vspace{-0.1cm}
% % and evaluated on the same bias severity setting (1.0\%).}
% \resizebox{1.0\linewidth}{!}{
% \setlength{\tabcolsep}{0.7em}
% % \def\arraystretch{1.2}% 
% \begin{tabular}{ c | c c | c c}
% % \hline\noalign{\smallskip}
% \toprule 

% % Method & $\rho$ & $M$ & Colored MNIST & BFFHQ & Dogs \& Cats & BAR \\
% % \multicolumn{1}{c|}{\multirow{2}{*}{Method}}
% % \multicolumn{1}{c}{\multirow{2}{*}{$\rho$}}
% \multicolumn{1}{c|}{\multirow{2}{*}{}}

% % & $\mathcal{D}_\text{C}$  & \multicolumn{2}{c}{$\mathcal{D}_\text{aux}$}
% % & $\mathcal{D}_\text{C}$  & \multicolumn{2}{c}{$\mathcal{D}_\text{aux}$} 
% % \\ \cmidrule(lr){2-2} \cmidrule(lr){3-4} \cmidrule(lr){5-5} \cmidrule(lr){6-7}
% & \multicolumn{2}{c}{\# of B.A. $\downarrow$} 
% & \multicolumn{2}{c}{\# of B.C. $\uparrow$} 
% \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5}

% Dataset   
% % & {\# of B.A. $\downarrow$}
% % & {\# of B.A. $\downarrow$}
% % & {\% of B.A. $\downarrow$}
% % & {\# of B.C. $\uparrow$}
% % & {\# of B.C. $\uparrow$}
% % & {\% of B.C. $\uparrow$}
% & $\mathcal{D}_\text{C}$
% & $\mathcal{D}_\text{aux}$
% & $\mathcal{D}_\text{C}$
% & $\mathcal{D}_\text{aux}$

% \\
% \midrule
% Waterbirds 
% & 163.8\stdv{20.56}
% & 134.4\stdv{15.35}

% & 39.0\stdv{1.41}
% & 38.0\stdv{1.67}
% \\

% BFFHQ 
% & 286.8\stdv{47.57}
% & 87.0\stdv{16.8}

% & 104.0\stdv{1.41}
% & 96.0\stdv{2.0}
% \\

% \bottomrule
% \end{tabular}}

% % \vspace{-0.5cm}
% \label{tab:auxcomposition}
% \end{table}



% \begin{table}[t!]
% \centering
% % \vspace{0.05cm}
% % \caption{
% % The remaining number of bias-aligned samples~(\# of B.A.) and bias-conflicting ones~(\# of B.C.) in the bias-amplified dataset $\mathcal{D}_A$ after applying BE.
% % % $M$ indicates the number of BCDs.
% % The remaining numbers are shown in ratios of samples compared to the original training dataset $\mathcal{D}$.}
% \caption{The number of remaining bias-aligned samples (\# of B.A.) and bias-conflicting ones~(\# of B.C.) depending on sampling methods. The last column of each dataset represents the ratio of \# of B.A. to \# of B.C. }
% % \vspace{-0.1cm}
% % and evaluated on the same bias severity setting (1.0\%).}
% \resizebox{1.0\linewidth}{!}{
% \setlength{\tabcolsep}{0.7em}
% % \def\arraystretch{1.1}% 
% \begin{tabular}{ c | c c | c c}
% % \hline\noalign{\smallskip}
% \toprule 

% % Method & $\rho$ & $M$ & Colored MNIST & BFFHQ & Dogs \& Cats & BAR \\
% % \multicolumn{1}{c|}{\multirow{2}{*}{Method}}
% % \multicolumn{1}{c}{\multirow{2}{*}{$\rho$}}
% \multicolumn{1}{c|}{\multirow{2}{*}{}}

% & \multicolumn{2}{c}{Waterbirds}
% & \multicolumn{2}{c}{BFFHQ}
% \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5}
% & {\% of B.A. $\downarrow$}
% & {\% of B.C. $\uparrow$}
% & {\% of B.A. $\downarrow$}
% & {\% of B.C. $\uparrow$}
% \\
% \midrule
% $\mathcal{D}_\text{aux}$  
% & 2.83\stdv{0.32}
% & 0.45\stdv{0.08}
% & 79.1\stdv{3.48}
% & 50.0\stdv{1.04}
% \\

% \bottomrule
% \end{tabular}}

% % \vspace{-0.5cm}
% \label{tab:auxcomposition}
% \end{table}

==> table/mainresult.tex <==

\begin{table*}
\begin{center}
\caption{Image classification accuracy on test sets. We present the results with four different ratios of bias-conflicting samples. 
For the \textit{cross} and \textit{check} marks, the former indicates whether the model uses bias labels during training and the latter shows whether the model requires a predefined bias type.
The best accuracy values are in bold. Results with standard deviations are provided in the Supplementary.}
% \vspace{-0.3cm}
\resizebox{1.0\linewidth}{!}{
\setlength{\tabcolsep}{0.4em}
\def\arraystretch{1.1}% 
\begin{tabular}{ccccccccccccc}
% \hline\noalign{\smallskip}
\toprule 
\multirow{2.5}{*}{\large Dataset} 
& \multirow{2.5}{*}{\large Ratio (\%)} 
% & \multirow{2.5}{*}{\large Ratio} 
&
& Vanilla~\cite{He2015resnet}
& HEX~\cite{wang2018hex}
& LNL~\cite{kim2019LNL}
& EnD~\cite{EnD}
& ReBias~\cite{bahng2019rebias}
& LfF~\cite{nam2020learning}
& DE~\cite{disentangled}
& LfF*~\cite{lee2022revisiting}
& DE*~\cite{lee2022revisiting}
& Ours
% & xx
% & xx
% & xx
% & xx
% & xx
% & xx
% & xx
% & xx
% & xx
% & xx
\\

\cmidrule{4-13}
&&
& \textcolor{black}{\boldxmark} \textcolor{black}{\boldxmark}
& \textcolor{black}{\boldxmark} \textcolor{black}{\boldcheckmark}
& \textcolor{black}{\boldcheckmark} \textcolor{black}{\boldcheckmark}
& \textcolor{black}{\boldcheckmark} \textcolor{black}{\boldcheckmark}
& \textcolor{black}{\boldxmark} \textcolor{black}{\boldcheckmark}
& \textcolor{black}{\boldxmark} \textcolor{black}{\boldxmark}
& \textcolor{black}{\boldxmark} \textcolor{black}{\boldxmark}
& \textcolor{black}{\boldxmark} \textcolor{black}{\boldxmark}
& \textcolor{black}{\boldxmark} \textcolor{black}{\boldxmark}
& \textcolor{black}{\boldxmark} \textcolor{black}{\boldxmark}
\\

\midrule
\multirow{4}{*}{CMNIST}
 % xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
 % xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
 % xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
 % xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\

& 0.5 & & 79.07 & 14.70 & 76.33 & 78.65 & 67.47 & 92.75 & 78.99 & 93.07 & 92.03 & \textbf{95.20} \\
& 1.0 & & 88.91 & 25.66 & 88.51 & 89.07 & 82.55 & 95.12 & 89.46 & 95.13 & 94.50 & \textbf{96.50} \\
& 2.0 & & 93.92 & 30.14 & 92.94 & 93.80 & 90.64 & 95.32 & 92.38 & 96.65 & 96.23 & \textbf{97.29} \\
& 5.0 & & 96.92 & 78.04 & 96.43 & 96.82 & 95.66 & 96.38 & 95.85 & 97.75 & 97.43 & \textbf{98.26} \\


\midrule
\multirow{4}{*}{Waterbirds}
& 0.5 & & 56.12 & 55.74 & 56.59 & 55.85 & 54.85 & 59.62 & 57.92 & 59.31 & 59.53 & \textbf{63.12} \\
& 1.0 & & 56.69 & 56.36 & 56.83 & 56.47 & 55.71 & 59.50 & 59.16 & 59.96 & 59.14 & \textbf{61.89} \\
& 2.0 & & 58.33 & 58.81 & 59.26 & 58.80 & 56.29 & 59.29 & 60.39 & 58.63 & 56.78 & \textbf{64.14} \\
& 5.0 & & 60.75 & 61.05 & 63.31 & 60.72 & 58.38 & 56.49 & 60.45 & 58.69 & 58.54 & \textbf{64.36} \\

\midrule
\multirow{4}{*}{BFFHQ}
& 0.5 & & 55.64 & 56.96 & 56.88 & 55.96 & 55.76 & 65.19 & 62.08 & 67.36 & 67.56 & \textbf{70.84} \\
& 1.0 & & 60.96 & 62.32 & 62.64 & 60.88 & 60.68 & 69.24 & 66.00 & 75.08 & 73.48 & \textbf{78.84} \\
& 2.0 & & 69.00 & 70.72 & 69.80 & 69.72 & 69.60 & 73.08 & 69.92 & 80.32 & 79.48 & \textbf{83.64} \\
& 5.0 & & 82.88 & 83.40 & 83.08 & 82.88 & 82.64 & 79.80 & 80.68 & 85.48 & 84.84 & \textbf{87.64} \\

\midrule
\multirow{2}{*}{BAR}
& 1.0 & & 60.96 & 62.32 & 62.64 & 60.88 & 60.68 & 69.24 & 66.00 & 75.08 & 73.48 & \textbf{78.84} \\
& 5.0 & & 82.88 & 83.40 & 83.08 & 82.88 & 82.64 & 79.80 & 80.68 & 85.48 & 84.84 & \textbf{87.64} \\


\bottomrule

\end{tabular}
}
% \vspace{-0.8cm}
\label{tab:best_test}
\end{center}
\end{table*}
